Multi-step Entity-centric Information Retrieval for Multi-Hop Question Answering

Multi-hop question answering (QA) requires an information retrieval (IR) system that can find \emph{multiple} supporting evidence needed to answer the question, making the retrieval process very challenging. This paper introduces an IR technique that uses information of entities present in the initially retrieved evidence to learn to `\emph{hop}' to other relevant evidence. In a setting, with more than \textbf{5 million} Wikipedia paragraphs, our approach leads to significant boost in retrieval performance. The retrieved evidence also increased the performance of an existing QA model (without any training) on the \hotpot benchmark by \textbf{10.59} F1.

==> Information Retrieval for Multi-Hop Question Answering/sections/experiments.tex <==
\section{Experiments}
For all our experiment, unless specified otherwise, we use the open domain corpus\footnote{\url{https://hotpotqa.github.io/wiki-readme.html}} released by \citet{yang2018hotpotqa} which contains over 5.23 million Wikipedia abstracts (introductory paragraphs). To identify spans of entities, we use the implementation of the state-of-the-art entity tagger presented in \citet{peters2018deep}.\footnote{\url{https://allennlp.org/models}} For the \bert encoder, we use the \textsc{Bert-base-uncased} model.\footnote{\url{https://github.com/google-research/bert}} We use the implementation of widely-used \bm retrieval available in Lucene.\footnote{\url{https://lucene.apache.org/}} 

% Although, the main goal of our work is to improve retrieval performance for multi-hop QA, we find that our simple entity linker works quite well in practice with an accuracy of 91.1\%. The highest scoring entity paragraphs for each mentions, are then passed to the retriever for re-ranking.
% For every query, we consider the top \raj{xx} paragraphs retrieved by Lucene.  
% Our method introduces a new way of doing multi-step retrieval in which new evidence are searched based on the set of initially retrieved evidence. A popular way of doing it in traditional IR  systems is via psuedo-relevance feedback (\textsc{Prf}). The PRF methods depend on a relevance model that decides which terms are relevant for reformulating the query. We compare with two widely used PRF techniques --- based on term-frequency (\textsc{Prf-tfidf}) \cite{xu2017quary} and on language model (\textsc{Prf-lm}) \cite{lavrenko2017relevance}. \citet{nogueira2017task} recently proposed a new way of query reformulation incorporating performance incproporating reward from a  document relevance task (\textsc{Prf-task}) and training using reinforcement learning. 

 

\subsection{IR for MultiHop QA}
We introduce a new way of doing multi-step retrieval. A popular way of doing it in traditional IR systems is via pseudo-relevance feedback (\textsc{Prf}). The \prf methods assume that the top retrieved documents in response to a given query are relevant. Based on this assumption, they expand the query in a weighted manner. \prf has been shown to be effective in various retrieval settings~\cite{xu2017quary}. We compare with two widely used \prf models  --- The Rocchio's algorithm on top of the TF-IDF retrieval model (\textsc{Prf-tfidf}) \cite{Rocchio:1971} and the relevance model (RM3) based on the language modeling framework in information retrieval (\textsc{Prf-rm}) \cite{lavrenko2017relevance}. Following prior work~\cite{nogueira2017task}, we use query likelihood retrieval model with Dirichlet prior smoothing \cite{zhai2017study} for first retrieval run. 

\citet{nogueira2017task} proposed a new way of query reformulation --- incorporating reward from a document-relevance task (\textsc{Prf-task}) and training using reinforcement learning. 
% We use the open source implementation released by the authors. 
Recently, \citet{nogueira2019passage} proposed a \bert based passage re-ranker (\bert-re-ranker) that has achieved excellent performance in several IR benchmarks. 
But, its performance has not been evaluated on multi-hop queries till now. 
For a fair comparison with our model which looks at paragraphs corresponding to entities, we use top 200 paragraphs retrieved by the initial IR model for \bert-re-ranker instead of 25 for our model.\footnote{There were 2.725 entities in the paragraph on average}

\begin{table}
    \small
    \centering
    \begin{tabular}{@{} l c c c c c @{}}\toprule
    & \multicolumn{4}{c}{\textsc{Accuracy}  } & \\
    \cline{2-5}\noalign{\smallskip}
    Model & @2 & @5 & @10 & @20 & \textsc{map} \\\midrule
    \bm & 0.093 & 0.191 & 0.259&  0.324 & 0.412\\
    \textsc{Prf-tfidf} & 0.088 & 0.157 & 0.204  & 0.258 & 0.317\\
    \textsc{Prf-rm}  & 0.083 & 0.175 & 0.242 & 0.296 & 0.406\\ 
    \textsc{Prf-task}  & 0.097 & 0.198 & 0.267 & 0.330 & 0.420\\\midrule
    \bert-re-ranker & 0.146 & 0.271 & 0.347 & 0.409 & 0.470\\
    \textsc{Query+E-doc} & 0.101 & 0.223 & 0.301 & 0.367 & 0.568\\
    % \textsc{Query-indep.} & 0.023 & 0.094  & 0.279 & 0.519 & - \\
    \midrule
    Our Model &\textbf{0.230} & \textbf{0.482}&  \textbf{0.612}& \textbf{0.674} & \textbf{0.654}\\\bottomrule
    \end{tabular}
    \caption{Retrieval performance of models on the \hotpot benchmark. A successful retrieval is when \emph{all} the relevant passages for a question are retrieved from more than 5 million paragraphs in the corpus.}
    \label{tab:retriever}
    \vspace{-3mm}
\end{table}

Table~\ref{tab:retriever} reports the accuracy(@$k$) of retrieving \emph{all} the relevant paragraphs required for answering a question in \hotpot.\footnote{Since, the supporting passage information is only present for train \& validation set, we consider the validation set as our hidden test set and consider a subset of train as validation set.} We compare the supporting passage annotation present in the dataset with the retrieved paragraph and retrieval is only correct when all the supporting paragraphs are in the top $k$ retrieved passages. We also report the mean average precision score (\textsc{map}) which is a strict metric that takes into account the relative position of the relevant document in the ranked list \cite{kadlec2017knowledge}. As we can see, our retrieval technique vastly outperforms other existing retrieval systems with an absolute increase of \textbf{26.5}\% (accuracy@10) and \textbf{18.4}\% (\textsc{map}), when compared to \bert-re-ranker. The standard \prf techniques do not perform well for this task. This is primarily because the \prf methods rely on statistical features like frequency of terms in the document, and fail to explicitly use information about entities, that may not be frequently occurring the paragraph. In fact, their performance is a little behind the standard retrieval results of \bm, suggesting that this benchmark dataset needs entity-centric information retrieval. The \textsc{Prf-task} does slightly better than other \prf models, showing that incorporating task-specific rewards can be beneficial. However, as we find, RL approaches are slow to converge\footnote{Training took $\sim$2 weeks for comparable performance.} as rewards from a down-stream tasks are sparse and action space in information retrieval is very large.\\
\textbf{Ablations}. We investigate whether modeling the chain of paragraphs needed to reach the final paragraph is important or not. As an ablation, we ignore the representation of the initial retrieved document $\mathrm{D}_1$ and only consider the final document representing the entity (\textsc{Query+E-doc}). Table~\ref{tab:retriever} shows that, indeed modeling the chain of documents is important. This makes intuitive sense, since to answer questions such as the county where a person is from (figure~\ref{fig:multi_hop_ex1}), modeling context about the person, should be helpful.
We also evaluate, if our model performs well on single-hop questions as well. This evaluation is a bit tricky to do in \hotpot, since the evaluataion set only contains questions from `hard' subset \cite{yang2018hotpotqa}. However, within that hard subset, we find the set of question, that has the answer span present in \emph{all} the supporting passages (\textsc{single-hop (hard)}) and only in \emph{one} of the supporting passages (\textsc{multi-hop (hard)})\footnote{There were 1184 \textsc{single-hop (hard)} and 4734 \textsc{multi-hop (hard)} queries.}. The intuition is that if there are multiple evidence containing the answer spans then it might be a little easier for a downstream QA model to identify the answer span. Figure~\ref{fig:single_vs_multi} shows that our model performs equally well on both type of queries and hence can be applied in a practical setting.
\begin{figure}
    \centering
    \vspace{-2mm}
    \includegraphics[width=0.7\columnwidth]{images/multi_hop_baseline.pdf}
    \vspace{-3mm}
    \caption{Our retrieval model works equally well for single-hop queries. This can be attributed to the presence of self-loops in the model which can make the model not hop to a different paragraph, if not required.}
    \label{fig:single_vs_multi}
    \vspace{-3mm}
\end{figure}
\subsection{Performance on \hotpot}
Table~\ref{tab:QA} shows the performance on the QA task. We were able to achieve better scores than reported in the baseline reader model of \citet{yang2018hotpotqa} by using Adam \cite{kingma2014adam} instead of standard SGD (our re-implementation). Next, we use the top-10 paragraphs retrieved by our system from the entire corpus and feed it to the reader model. We achieve a \textbf{10.59} absolute increase in F1 score than the baseline. It should be noted that we use the simple baseline reader model and we are confident that we can achieve better scores by using more sophisticated reader architectures, e.g. using \bert based architectures. 
Our results show that retrieval is an important component of an open-domain system and equal importance should be given to both the retriever and reader component.
\begin{table}
    \small
    \centering
    \begin{tabular}{@{} l c c @{}}\toprule
    Model & EM & F1   \\\midrule
    Baseline Reader \cite{yang2018hotpotqa} & 23.95 & 32.89\\
    Our re-implementation & 26.06 & 35.67 \\  
      + retrieved result &\textbf{35.36} & \textbf{46.26} \\\bottomrule
    \end{tabular}
    \caption{Performance on QA task on hidden test set of \hotpot after adding the retrieved paragraphs}
    \label{tab:QA}
    \vspace{-3mm}
\end{table}
\subsection{Zero-shot experiment on Wikihop}
We experiment if our model trained on \hotpot can generalize to another multi-hop dataset -- \whop \cite{welbl2018constructing}, without any training. In the \whop dataset, a set of candidate introductory Wikipedia paragraphs are given per question. Hence, we do not need to use our initial \bm retriever.

We assign the first entity mention occurring in a paragraph as the textual description of that entity. For instance, if the first entity mention in the paragraph is `Mumbai', we assign that paragraph as the textual description for the entity `Mumbai'. This assumption is often true for the introductory paragraphs of a Wikipedia article. Next, we perform entity linking of mentions by just simple string matching (i.e. linking strings such as `mumbai' to the previous paragraph). After constructing a small subgraph from the candidate paragraphs, we apply our model trained on \hotpot. The baseline models we compare to are a \bm retriever and a \bert-re-ranker model of \citep{nogueira2019passage} that ranks all the candidate supporting paragraphs for the question. Table~\ref{tab:wikihop} shows our model outperforms both models in zero-shot setting.

\begin{table}
    \small
    \centering
    \begin{tabular}{@{} l c c @{}}\toprule
    Model & acc@2 & acc@5   \\\midrule
    \bm & 0.06 & 0.30\\
    \bert-re-ranker (zs) & 0.08 & 0.27 \\  
    Our Model (zs) &\textbf{0.10} & \textbf{0.41} \\\bottomrule
    \end{tabular}
    \caption{Zero-shot (zs) IR results on \whop.}
    \label{tab:wikihop}
    \vspace{-3mm}
\end{table}


%Since the number of paragraphs is small for each question, the initial retriever selects only two documents and the re-ranker ranks the outgoing entities.
% \subsection{Zero-shot \whop experiment}
% \raj{Incomplete}. In this experiment, we plan to show a model trained on the \hotpot can be applied without any training to \whop dataset. Experiments ongoing.
% \subsection{\complex experiment}
% \raj{Incomplete}. Here the corpus is web snippets returned by Google. So we are doing cross-document co-reference to get links. Experiments ongoing.






% \begin{itemize}
%     \item PRF and its variants based on LMs and embeddings
%     \item Query reformulation using RL (Rodriguez model)
%     \item BERT re-ranker --- this is important and afaik, we dont have these numbers yet. 
% \end{itemize}

% \subsection{Results on open-domain \hotpot setting}
% \subsubsection{Results using gold entity links in the wikipedia paragraph}
% \raj{This is already done and we have significant improvements over baseline}

% \subsubsection{Results without entity links}
% Ameya is working on this with high priority. The goal of this experiment is to show that we are not dependent on the entity links. The baseline here would be neural BERT re-ranker ((if they are easy to apply)

% \subsection{Results on \whop zero-shot setting}
% Use the trained model on open domain setting and apply it here. Once again the baseline here would be a BERT re-ranker and PRF (if they are easy to apply)

% \subsection{Results on \complex }
% This experiment is to show that we are not restricted to just Wikipedia domain. \complex contains web snippets returned by Google which dont have entity links. So here we have to cross-doc coreference. To be honest, this experiment is tricky to do, because this will depend a lot on the coreference cluster. So I am a little worried about this experiement.

% \subsection{Results on QA}
% This is straightforward and we show improvements on a QA task by incorporating paragraphs retrieved from our reader. I am close to getting results on this one.




==> Information Retrieval for Multi-Hop Question Answering/sections/intro.tex <==
\section{Introduction}

Multi-hop QA requires finding multiple supporting evidence, and reasoning over them in order to answer a question \cite{welbl2018constructing,talmor2018web,yang2018hotpotqa}. For example, to answer the question shown in figure~\ref{fig:multi_hop_ex1}, the QA system has to retrieve two different paragraphs and reason over them. Moreover, the paragraph containing the answer to the question has very little lexical overlap with the question, making it difficult for search engines to retrieve them from a large corpus. For instance, the accuracy of a \bm retriever for finding \emph{all} supporting evidence for a question decreases from 53.7\% to 25.9\% on the `easy' and `hard' subsets of the \hotpot training dataset.\footnote{According to \citet{yang2018hotpotqa}, the easy (hard) subset primarily requires single (multi) hop reasoning. We only consider queries that have answers as spans in at least one paragraph.}


We hypothesize that an effective retriever for multi-hop QA should have the ``\emph{hopiness}'' built into it, by design. That is, after retrieving an initial set of documents, the retriever should be able to ``hop'' onto other documents, if required. We note that, many supporting evidence often share common (\emph{bridge}) entities between them (e.g. ``Rochester Hills'' in figure~\ref{fig:multi_hop_ex1}). In this work, we introduce a model that uses information about entities present in an initially retrieved paragraph to jointly find a passage of text \emph{describing} the entity (\emph{entity-linking}) and also determining whether that passage would be relevant to answer the multi-hop query.

% present in a initially retrieved paragraph to determine if documents describing those entities would be more relevant to answer the question. 

%In a large scale open domain setting, containing over 5,000,000 Wikipedia documents, we show that our retriever is able to improve over the accuracy of retrieving all supporting evidence over a widely used baseline retrieval system by 34 absolute points. 
\begin{figure}
    \centering
    \vspace{-2mm}
    \includegraphics[width=\columnwidth]{images/MultihopQA-example-crop.pdf}
    \caption{Multi-hop questions require finding multiple evidence and the target document containing the answer has very little lexical overlap with the question.}
    \label{fig:multi_hop_ex1}
    \vspace{-3mm}
\end{figure}

% At a high level, our retrieval mechanism works as follows --- The query is initially fed into a standard IR system (e.g. \bm) that returns an initial set of evidence. In our preliminary experiments, we find that this initial evidence set often covers the entities in the query (e.g. the paragraph corresponding to Ron Teachworth in figure~\ref{fig:multi_hop_ex1}). However, to answer multi-hop questions, we need to gather more evidence. 

A major component of our retriever is a re-ranker model that uses contextualized entity representation obtained from a pre-trained \bert \cite{devlin2018bert} language model. Specifically, the entity representation is obtained by feeding the query and a Wikipedia paragraph describing the entity to a \bert model. The re-ranker uses representation of both the initial paragraph and the representation of all the entities within it to determine which evidence to gather next. 

% The document describing the entity can be obtained by following the anchor links present in the Wikipedia document. However, for our approach to be more generally applicable, we also train an entity linker to identify the corresponding Wikipedia page from the mention of an entity. Further, to demonstrate that we are not restricted to just the Wikipedia domain, we experiment in a setting where the evidence set comprises of web search results. Finding entity links now corresponds to doing cross-document entity linking \cite{bagga1998entity,rao2010streaming} within the set of evidence and we show that our model can be effectively applied to this setting as well. 

\begin{figure*}
\centering
    \includegraphics[width=1.75\columnwidth]{images/Entity_Centric_IR-crop.pdf}
\caption{Overview of our approach. We use the entity mentions present in the initially retrieved paragraphs to link to paragraphs describing them. Next, the \bert-based re-ranker scores the chain of initial and the entity-describing paragraph. Note the presence of self-loop from the initial paragraphs to accommodate for questions that do not require `hopping' to a new paragraph.}
\label{fig:model}
\end{figure*}
Essentially, our method introduces a new way of \emph{multi-step} retrieval that uses information about intermediate entities. 
A standard way of doing multi-step retrieval is via \emph{pseudo-relevance feedback} \cite{xu2017quary,lavrenko2017relevance} in which relevant terms from initial retrieved documents are used to reformulate the initial question. A few recent works learn to reformulate the query using task specific reward such as document recall or performance on a QA task \cite{nogueira2017task,buck2017ask,das2018multi}. However, these methods do not necessarily use the information about entities present in the evidence as they might not be the more frequent/salient terms in it. Empiricially, our method outperforms all of these methods significantly for multi-hop QA. Our work is most closely related to the recently proposed \bert re-ranker model of \citet{nogueira2019passage}. However, unlike us, they do not model the chains of evidence paragraphs required for a multi-hop question. Secondly, they also do not have a entity linking component to identify the relevant paragraphs. Our model out-performs them for multi-hop QA.

% To summarize, this paper makes the following contributions --- (a) We present an entity-centric IR approach that effectively finds relevant evidence required for questions that need multi-hop reasoning from a large corpus containing millions of paragraphs. When the retrieved paragraphs are supplied to the baseline QA model introduced in \citet{yang2018hotpotqa}, it improved the QA performance by 4.5 F1 points. (b) We also show that our model is not restricted to only Wikipedia domain and can be applied to generic web search results.

To summarize, this paper presents an entity-centric IR approach that jointly performs entity linking and effectively finds relevant evidence required for questions that need multi-hop reasoning from a large corpus containing millions of paragraphs. When the retrieved paragraphs are supplied to the baseline QA model introduced in \citet{yang2018hotpotqa}, it improved the QA performance on the hidden test set by 10.59 F1 points.\footnote{Code, pre-trained models and retrieved paragraphs are released --- \url{https://github.com/ameyagodbole/entity-centric-ir-for-multihop-qa}}
% (b) We also show that our model is not restricted to only Wikipedia domain and can be applied to generic web search results.

% (b) We show that our model trained on the \hotpot dataset can be applied without \emph{any training} to the \whop dataset. Furthermore, we show that our model can be also applied to generic web-search results and is not restricted to just the Wikipedia domain. (c) Lastly, we show that the paragraphs retrieved by our model,  when supplied to the baseline reader introduced in \citet{yang2018hotpotqa} for \hotpot dataset leads to significant improvement in the open-domain setting.

% \raj{Motivate some more why entity centric information retrievel is important. Cite some papers here as well. @Hamed, are there any IR papers which give importance to entities?. I think here we should also mention that we use BERT embeddings,  and also that we show impropvements on both cases where we see gold entity links and when we dont.}
% The contributions of our paper are as follows --- (a) We present a novel entity-centric information retrieval technique that effectively finds relevant evidence for questions requiring multi-hop reasoning from a large corpus containing millions of Wikipedia paragraphs. We demonstrate that our method trained in the open-domain setting on the \hotpot dataset can be used in zero-shot settings to the \whop dataset. We additionally show that our retriever can be applied to web search results demonstrating that our technique is not restricted to the Wikipedia domain. (c) Lastly, we show \raj{significant} improvements in a downstream QA task by using the results from our entity-centric multi-hop retriever. 



% We note that the supporting evidence often share common (\emph{bridge}) entities between them (e.g. ``Rochester Hills, Michigan'' in figure 1). In this work, we introduce a model that uses information about entities present in a initially retrieved document to determine if documents describing the entities would be more relevant to answer the question. 

% to augment the initial set of evidence retrieved by a search engine in the initial step. This augmented set of evidence is then re-ranked by a model that uses contextualized representation of entities to determine the target evidence. Specifically, 

==> Information Retrieval for Multi-Hop Question Answering/sections/methodology.tex <==
\section{Methodology}
\label{sec:model}
Our approach is summarized in Figure~\ref{fig:model}. The first component of our model is a standard IR system that takes in a natural language query `$\mathrm{Q}$' and returns an initial set of evidence. For our experiments, we use the popular \bm retriever, but this component can be replaced by any IR model. We assume that all spans of entity mentions have been identified in the paragraph text by a one-time pre-processing, with an entity tagger.\footnote{We plan to explore joint learning of entity tagging with linking and retrieval as future work.}
% Next we describe the \bert based ranking model that scores each outgoing entity links in the initial document. \\

\paragraph{Entity Linking} The next component of our model is an entity linker that finds an introductory Wikipedia paragraph describing the entity, corresponding to each entity mention. Several IR approaches \cite{xiong2016bag,raviv2016document} use an off-the-shelf entity linker. However, most entity linking systems \cite{ganea,raiman2018deeptype} have been trained on Wikipedia data and hence using an off-the-shelf linker would be unfair, since there exists a possibility of test-time leakage. To ensure strictness, we developed our own simple linking strategy. Following the standard approach of using mention text and hyper-link information \cite{cucerzan2007large,ji2011knowledge}, we create a mapping (alias table) between them. The alias table stores mappings between a mention string (e.g. ``Bill'') and various entities it can refer to (e.g. Bill Clinton, Billy Joel, etc).
The top-40 documents returned by the \bm retriever on the dev and test queries are also ignored while building the alias table.
At test time, our re-ranker considers all the candidate entity paragraphs that a mention is linked to via the alias table. Although simple, we find this strategy to work well for our task and we plan to use a learned entity linker for future work.

%To ensure fairness, while building the alias table, we ignore the top-40 documents returned by the \bm retriever on the dev and test queries.

% Next, we train a simple linker that learns to identify the correct Wikipedia entity paragraph by using the contextualized representation of the mention string and the text in the paragraph describing the entity. Let $\mathrm{e}$ be an entity mention in $\mathrm{D_1}$ that is linked to its corresponding wikipage $\mathrm{E}.$ To get the mention and entity representation, we encode $\mathrm{D_1}$ and $\mathrm{E}$ with a \bert encoder. The mention representation  correspond to the token level representation of the last layer obtained from \bert encoder. We average the token representation for multi-word entities. For the entity representation, we consider the representation corresponding to the \cls token in $\mathrm{E}$. The \cls token representation has commonly been used for many document level classification tasks \cite{devlin2018bert} and also for passage re-ranking \cite{nogueira2019passage}. In a practical scenario, most queries to a IR system will not be multi-hop in nature. To account for such cases, we also add a \emph{self-link} from each document to itself. This allows the model to remain in the same document, if necessary. The score between a mention and entity representation is computed by concatenating both representation and passing it through a two-layer feed-forward network to output a score. During training, we use entries in the alias table mappings as positive examples and we use randomly sampled entity paragraphs as negative samples. The network is trained to minimize the cross-entropy loss. 

\paragraph{Re-ranker} The next component of our model is a \bert-based re-ranker that ranks the chains of paragraphs obtained from the previous two components of the model. Let $\mathrm{Q}$ denote the query, $\mathrm{D}$ denote a paragraph in the initial set of paragraphs returned by the \bm retriever. Let $\mathrm{e}$ denote an entity mention present in $\mathrm{D}$ and $\mathrm{E}$ be the linked document returned by the linker for $\mathrm{e}$. If there are multiple linked documents, we consider all of them. Although our retriever is designed for multi-hop questions, in a general setting, most questions are not multi-hop in nature. Therefore to account for questions that do not need hopping to a new paragraph, we also add a `self-link' (Figure~\ref{fig:model}) from each of the initial retrieved paragraph, giving the model the ability to stay in the same paragraph.

To train the re-ranker, we form \emph{query-dependent} passage representation for both $\mathrm{D}$ and $\mathrm{E}$. The query $\mathrm{Q}$ and the paragraph $\mathrm{E}$ are concatenated and fed as input to a \bert encoder and the corresponding \cls token forms the entity representation $\mathbf{e}$. Similarly, the document representation $\mathbf{d}$ is set to the embedding of the \cls token obtained after encoding the concatenation of $\mathrm{Q}$ and $\mathrm{D}$. The final score that the entity paragraph $\mathrm{E}$ is relevant to $\mathrm{Q}$ is computed by concatenating the two query-aware representation $\mathbf{d}$ and $\mathbf{e}$ and passing it through a 2-layer feed-forward network as before. It should be noted, the final score is determined by both the evidence paragraphs $\mathrm{D}$ and $\mathrm{E}$ and as we show empirically, not considering both leads to decrease in performance.

During training, we mark a chain of paragraphs as a positive example, if the last paragraph of the chain is present in the supporting facts, since that is a chain of reasoning that led to a relevant paragraph. All other paragraph chains are treated as negative examples. In our experiments, we consider chains of length 2, although extending to longer chains is straightforward. We use a simple binary cross-entropy loss to train the network.

% The underlying \bert encoder is shared between the entity linker and retriever and is fine-tuned. The final loss is computed by simple addition of the losses from the two networks.


% \textbf{(a)} The query $\mathrm{Q}$ and the paragraph describing the entity $\mathrm{E}$ are concatenated and fed as input to a \bert encoder. Then the representation corresponding to the \cls token is used as the entity representation. The \cls token representation has commonly been used for many document level classification tasks \cite{devlin2018bert} and also for passage re-ranking \cite{nogueira2019passage}.
% After obtaining the entity representation $\mathbf{e}$, we need to score how likely, document $\mathrm{E}$ is going to answer $\mathrm{Q}$. This score is computed based on the query $\mathrm{Q}$, the initial document $\mathrm{D_1}$ and the document describing the entity $\mathrm{E}$. The document representation $\mathbf{d_1}$ is set to the embedding of the \cls token obtained after encoding the concatenation of $\mathrm{Q}$ and $\mathrm{D_1}$. The final scalar score is computed by concatenating the two query-aware document representation $\mathbf{d_1}$ and $\mathbf{e}$ and passing it through a 2-layer feed-forward network. \\
% \textbf{Entity Linking}. Till now, we assumed that we have access to the document describing an entity mention $\mathrm{e_i}$ in $\mathrm{D_1}$. Even though, this is a reasonable assumption in the Wikipedia setting, it will not generalize to other domains. 

% \textbf{(b)} In this encoder, instead of using the \cls representation, we identify the various entity mentions present in $\mathrm{E}$. The final entity representation is a weighted sum of all the entity mention representations occurring in $\mathrm{D_1}$. Let \{$\mathbf{e_1, e_2, \ldots, e_m}$\} be the set of entity mention representation in $\mathrm{E}$, where $\mathbf{e_i} \in \mathbb{R}^d$. These representation correspond to the token level representation of the last layer obtained from \bert encoder. For a mention containing multiple words, we average the individual token representation. The final entity representation $\mathbf{e}$ is obtained as follows
% \begin{align*}
%      a_i =& \frac{\exp(\mathbf{w^\top\mathbf{e}_{i}})}{\sum_{i'}{\exp(\mathbf{w}^\top \mathbf{e}_{i'})}} & \mathbf{e} =&\sum_{i'}a_{i'} \cdot \mathbf{e_{i'}}
% \end{align*}

% \textbf{Entity Representation and Scoring}. Let us assume that all entity mentions in an initially retrieved document $\mathrm{D_1}$ have been identified and linked to their corresponding Wikipedia pages. Let $\mathrm{e}$ be an entity mention in $\mathrm{D_1}$ that is linked to its corresponding wikipage $\mathrm{E}.$ We experiment with the following two entity encoders to compute entity representation $\mathbf{e} \in \mathbb{R}^d$. \\

==> Information Retrieval for Multi-Hop Question Answering/sections/related_work.tex <==
\section{Related Work}
\textbf{Document retrieval using entities}. Analysis of web-search query logs has revealed that there is a large portion of entity seeking queries \cite{liu2015latent}. There exists substantial work on modeling documents with entities occurring in them. For example, \citet{xiong2016bag} represents a document with bag-of-entities and \citet{raviv2016document} use entity-based language modeling for document retrieval. However, they depend on an off-the-shelf entity tagger, where as we jointly perform linking and retrieval. Moreover, we use contextualized entity representations using pre-trained LMs which have been proven to be better than bag-of-words approaches.
There has been a lot of work which leverages knowledge graphs (KGs) to learn better entity representations \cite{xiong2015esdrank,xiong2017word,liu2018entity} and for better query reformulation \cite{cao2008selecting,dalton2014entity,dietz2014umass}. Our work is not tied to any specific KG schema, instead we encode entities using its text description.  
\\
\textbf{Neural ranking} models have shown great potential and have been widely adopted in the IR community \cite[inter-alia]{dehghani2017nrm,guo:2019,mitra2017learning,zamani2018neural}. Bag-of-words and contextual embedding models, such as word2vec and BERT, have also been explored extensively for various IR tasks, from document to sentence-level retrieval~\cite{padigela2019,zamani2016emb,zamani2017relwe}.
% Apart from IR, modeling entities has helped language modeling \cite{ji2017dynamic} and text generation \cite{clark2018neural}. 
% and reading comprehension \cite{das2018building}.


% Recently, \citet{nogueira2019passage} proposed a \bert based re-ranker that has achieved excellent performance in passage-level IR benchmarks. This is the closest work to ours, but we learn to find evidence by entity linking and also model \emph{chains} of evidence relevant for multi-hop QA.\\
% \textbf{Entity linking}. \raj{incomplete}
% Neural ranking models have shown great potential in the IR community and several recent work has adopted them \cite{guo2016deep,mitra2017learning,hui2018co}. Recently, \citet{nogueira2019passage} propose a \bert based re-ranker that has achieved excellent performance in several IR benchmarks. But, its performance has not been evaluated on multi-hop queries till now. We compare with the \bert re-ranker model.

